Towards Relaxed Multimodal Inputs for Gait-based Parkinson's Disease Assessment

Parkinson's disease assessment has garnered growing interest in recent years, particularly with the advent of sensor data and machine learning techniques. Among these, multimodal approaches have demonstrated strong performance by effectively integrating complementary information from various data sources. However, two major limitations hinder their practical application: (1) the need to synchronize all modalities during training, and (2) the dependence on all modalities during inference. To address these issues, we propose the first Parkinson's assessment system that formulates multimodal learning as a multi-objective optimization (MOO) problem. This not only allows for more flexible modality requirements during both training and inference, but also handles modality collapse issue during multimodal information fusion. In addition, to mitigate the imbalance within individual modalities, we introduce a margin-based class rebalancing strategy to enhance category learning. We conduct extensive experiments on three public datasets under both synchronous and asynchronous settings. The results show that our framework-Towards Relaxed InPuts (TRIP)-achieves state-of-the-art performance, outperforming the best baselines by 16.48, 6.89, and 11.55 percentage points in the asynchronous setting, and by 4.86 and 2.30 percentage points in the synchronous setting, highlighting its effectiveness and adaptability.

==> samples/tables/dataset_stats.tex <==
\begin{table}[t]
\centering
\caption{Statistics of Multimodal PD Locomotive Datasets}
\label{tab:stats_dataset}
\renewcommand\arraystretch{1.2}{
\setlength{\tabcolsep}{.9 mm}{
\begin{adjustbox}{max width=\linewidth,center}
\begin{tabular}{cccc}
\hline
% \begin{tabular}[c]{@{}c@{}}Clinical \\ Scales\end{tabular}
Dataset 
& Sample Count & Class Count & Modalities \\ \hline

FOG~\cite{ribeiro2022public} & 1856 
% & 35 
& \begin{tabular}[c]{@{}c@{}}3 \\ (H\&Y Scale) \end{tabular} & \begin{tabular}[c]{@{}c@{}} IMU \\ Skeleton \end{tabular} \\ \hline

FBG~\cite{shida2023public} & 4462 
% & 26 
& \begin{tabular}[c]{@{}c@{}} 3 \\ (MDS-UPDRSIII) \end{tabular} & \begin{tabular}[c]{@{}c@{}} vGRF \\ Skeleton \end{tabular}     \\ \hline

WearGait~\cite{kontson2024wearables} & 5219
% & 183
& \begin{tabular}[c]{@{}c@{}}2 \\(PD or Healthy) \end{tabular} & \begin{tabular}[c]{@{}c@{}} Walkway \\ Insole, IMU \end{tabular}     \\ \hline

\end{tabular}
\end{adjustbox}
}
}
\end{table}


% \begin{table}[t]
%   \centering
%   \caption{Ablation accuracies and accuracy drops \(\Delta\) for sensor vs. skeleton modalities across fusion models.  
%   Each row lists the full-model accuracy and the accuracies when ablating (i.e. removing) one modality. Larger \(\Delta\) indicates that the modality is more indispensable.}
%   \label{tab:ablation-collapse}
%   \begin{adjustbox}{max width=\linewidth,center}
%   \begin{tabular}{lccccc}
%     \toprule
%     \multirow{1}{*}{Model} & Full Modality & w/o Sensor & w/o Skeleton & \(\Delta_{\text{sensor}}\) & \(\Delta_{\text{skeleton}}\)\\ 
%     % & (Acc\%) & (Acc\%) & (Acc\%) & (pp) & (pp) & \\ 
%     \midrule
%     Early Fusion   & 61.65 & 36.42 & 40.09 & 25.23 & 21.56 \\ 
%     Late Fusion    & 63.71 & 36.71 & 47.64 & 27.00 & 16.07 \\ 
%     Shared Latent  & 61.13 & 36.14 & 43.56 & 24.99 & 17.57 \\ 
%     \bottomrule
%   \end{tabular}
%   \end{adjustbox}
% \end{table}
